R&R: Metric-guided Adversarial Sentence Generation

Adversarial examples are helpful for analyzing and improving the robustness of text classifiers. Generating high-quality adversarial examples is a challenging task as it requires generating fluent adversarial sentences that are semantically similar to the original sentences and preserve the original labels, while causing the classifier to misclassify them. Existing methods prioritize misclassification by maximizing each perturbation's effectiveness at misleading a text classifier; thus, the generated adversarial examples fall short in terms of fluency and similarity. In this paper, we propose a rewrite and rollback (R&R) framework for adversarial attack. It improves the quality of adversarial examples by optimizing a critique score which combines the fluency, similarity, and misclassification metrics. R&R generates high-quality adversarial examples by allowing exploration of perturbations that do not have immediate impact on the misclassification metric but can improve fluency and similarity metrics. We evaluate our method on 5 representative datasets and 3 classifier architectures. Our method outperforms current state-of-the-art in attack success rate by +16.2%, +12.8%, and +14.0% on the classifiers respectively. Code is available at https://github.com/DAI-Lab/fibber

==> alg_advtrain.tex <==
\begin{algorithm*}[tb]
\SetAlgoLined
\KwIn{
Classifier $f(\bx)$;
Attack method $g(\bx, y, f)$ that creates a list of adversarial examples given a normal sentence, a label and a classifier;
Training set $\mathcal{D}=\{(\bx^{(i)}, y^{(i)})\}$;
Number of iterations $T$;
Number of attacks per iteration $t_1$;
Number of updates per iteration $t_2$;
Batch size $B$.}
\KwOut{Adversarially trained classifier $f(\cdot)$.}
$\texttt{reply\_buffer} = \{\}$\;
\For{$i$ in $1\ldots T$}{
    \For{$j$ in $1\ldots t_1$} {
        Sample $(\bx, y)\sim\mathcal{D}$\;
        \For {$\bu$ in $g(\bx, y, f)$} {
             $\texttt{reply\_buffer}.\texttt{add}((\bu, y))$;
        }
    }
    \For{$j$ in $1 \ldots t_2$} {
        Sample $\frac{B}{2}$ examples $\texttt{half\_batch\_normal}\sim \mathcal{D}$\;
        Sample $\frac{B}{2}$ examples $\texttt{half\_batch\_adv}\sim \texttt{reply\_buffer}$\;
        \For {$(\bu, y)$ in $\texttt{half\_batch\_adv}$} {
            $\texttt{reply\_buffer}.\texttt{delete}((\bu, y))$\;
        }
        Train $f$ with $\texttt{half\_batch\_normal} + \texttt{half\_batch\_adv}$\;
        \For {$(\bu, y)$ in  $\texttt{half\_batch\_adv}$} {
            \If {$f(\bu)\neq y$} {
                $\texttt{reply\_buffer}.\texttt{add}((\bu, y))$;
            }
        }
    }
}
\caption{Adversarial Training algorithm}\label{alg:advtrain}
\end{algorithm*}

==> alg_block.tex <==
\begin{algorithm*}[tb]
\SetAlgoLined
\KwIn{Original input $\bx=\{x_1,\ldots, x_l\}$; label $y$; Number of iterations $N$; Block size $m$.}
\KwOut{An adversarial example $\bu^{(N)}$.}
$R_\bx\leftarrow\sum_{t=1}^{l} E'(x_t)$\;

\For{$i$ in $1\ldots N$}{
    Randomly sample block starting position $st$ uniformly from $1\ldots l$\;
    $ed\leftarrow \min(st + m, l)$\;
    $\hat\bu^{(i)}\leftarrow\bu^{(i-1)}$\;
    
    \For{$k$ in $st\ldots ed$}{
        $\hat u^{(i)}_k\leftarrow\texttt{MASK}$;
    }
    \For {$k$ in $st\ldots ed$} {
        $R_\text{base}\leftarrow\sum_{t=1}^{l} E'(\hat u^{(i)}_t)\one[\hat u^{(i)}_t\neq \texttt{MASK}]$\;
        $p_\text{enforce}(z|\hat\bu^{(i)})\propto \exp(-w_\text{enforce}\max(0, \phi_\text{enforce}-\cos(R_\text{base} + E'(z), R_\bx)))$\;
        $p_\text{lm}\propto \text{BERT}(\hat\bu^{(i)})_k$\;
        Sample $z$ from $p_\text{proposal}(z|\hat\bu^{(i)})\propto p_\text{enforce}(z|\cdot)\times p_\text{lm}(z|\cdot)$\;
        $\hat u^{(i)}_k\leftarrow z$\;
    }
    Compute $\alpha=\frac{p_\text{target}(\hat\bu^{(i)}|\bx)}{p_\text{target}(\bu^{(i-1)}|\bx)}$\;
    $\bu^{(i)}=
    \begin{cases}
    \hat\bu^{(i)} & \text{ with probability } \alpha\\
    \bu^{(i-1)} & \text{otherwise}
    \end{cases}
    $\;
}
\caption{Block-sampling \model.}\label{alg:asrs}
\end{algorithm*}

==> alg_single.tex <==
\begin{algorithm}[htb]
\SetAlgoLined
\KwIn{Seed sentence $\bu^{(0)} = \{u_1^{(0)}, \ldots, u_l^{(0)}\};$ Number of iterations $N$.}
\KwOut{Rewritten sentence $\bu^{(N)}$.}
\For{$i$ in $1\ldots N$}{
    Sample $k^{(i)}$ uniformly from $1\ldots l$\;
    Compute $p_\text{proposal}(z|\bu^{(i-1)}_{-k^{(i)}})$ in Eq.~\eqref{eq:proposal}\;
    Sample $\hat z\sim p_\text{proposal}(z|\bu^{(i-1)}_{-k^{(i)}})$\;
    $\hat\bu^{(i)}\leftarrow \bu^{(i-1)}$; $\hat u^{(i)}_{k^{(i)}} \leftarrow \hat z$\;
    \uIf {$\text{decision}(\hat \bu^{(i)}, \bu^{(i-1)})=\text{Accept}$} {$\bu^{(i)}\leftarrow\hat\bu^{(i)}$\;}
    \Else {$\bu^{(i)}\leftarrow\bu^{(i-1)}$\;}
}
\caption{Single-word \framework.}\label{alg:single}
\end{algorithm}

==> table/notation.tex <==
\begin{table*}[htb]
    \centering
    \begin{tabular}{rp{10.5cm}}
        \toprule
        \textbf{Notation} & \textbf{Description}\\\midrule
        $(\mathbf{x}, y)$ &  One sentence and label pair, where $\mathbf{x}=\{x_1, x_2, \ldots, x_l\}$ is a sequence of $l$ words.\\
        $\Delta(\mathbf{x})$ & A set of sentences that are considered similar to $\mathbf{x}$.\\
        $\hat y = \arg\max f(\mathbf{x})$ & $f(\cdot)$ is a text classifier that outputs a distribution over all categories and $\hat y$ is the predicted label.\\
        $\mathbf{u}$ & A sampled sentence.\\
        $\text{ppl}(\cdot)$ & Perplexity of a sentence measured by GPT2 language model.\\
        $E(\cdot)$ & GloVe embedding table $E(x)\in\R^{300}$.\\
        $\cos(a, b)$ & the cosine similarity between two vectors $a$ and $b$.\\
        $R(\bx)$ & the GloVe embedding of a sentence.\\
        $H(\bx, \bu)$ & a transformer based sentence similarity metric.\\
        $w_\text{enforce}$ & the weight parameter for the enforcing distribution. \\
        $\phi_\text{enforce}$ & the threshold for the enforcing distribution. \\
        $w_\text{sim}$ & the weight parameter for the USE similarity term in the decision function. \\
        $\phi_\text{sim}$ & the threshold for the USE similarity term in the decision function. \\
        $w_\text{ppl}$ & the weight parameter for the GPT2 perplexity term in the decision function. \\
        $w_\text{ppl}$ & the weight parameter for the classifier term in the decision function. \\
        \bottomrule
    \end{tabular}
    \caption{Notations.}
    \label{tab:notation}
\end{table*}



==> table/table_ablation.tex <==
\begin{table*}[htb]
\centering
\small
\begin{tabular}{l|rrrrrr|rrrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{6}{c}{Dataset: AG} & \multicolumn{6}{c}{Dataset: MR}\\\cmidrule(lr){2-7}\cmidrule(lr){8-13}
\multicolumn{1}{c}{} & Acc\%  & USE  & CE   & PPL & Edit & \multicolumn{1}{c}{AR\%} & Acc\%  & USE  & CE   & PPL & Edit & \multicolumn{1}{c}{AR\%} \\\midrule
AG           & 10.0 & 0.82 & 0.88 & 1.0 & 12.7 & 26.2  & 1.0  & 0.76 & 0.93 & 1.2 & 8.9  & 29.0 \\
w/o enf.  & 13.0 & 0.81 & 0.89 & 1.1 & 12.2 & 23.8 & 1.0  & 0.74 & 0.91 & 1.0 & 8.6  & 22.5 \\
w/o dec. & 23.0 & 0.43 & 0.25 & 7.0 & 26.0 & N/A & 1.0  & 0.45 & 0.49 & 3.7 & 14.4 & N/A   \\
w/o clf.  & 67.0 & 0.79 & 0.88 & 0.9 & 12.6 & 28.3  & 37.0 & 0.75 & 0.91 & 0.8 & 10.9 & 33.3\\
w/o block & 41.0 & 0.84 & 0.90 & 1.0 & 8.1 & 76.1 & 18.0 & 0.79 & 0.92 & 1.1 & 6.6 & 81.2\\\bottomrule
\end{tabular}
\caption{Ablation study results of \modelc using the following metrics: after attack accuracy (Acc), USE and CE semantic similarity (USE/CE), GPT2 perplexity ratio (PPL),  edit distance (Edit) and acceptance rate in the decision function (AR).}\label{tab:ablation}
\vspace{-1ex}
\end{table*}


==> table/table_advtrain.tex <==
\begin{table*}[htb]
\small
\centering
\begin{tabular}{r|rrr|rrr}
\toprule
\multicolumn{1}{c}{Attack Method} & \multicolumn{3}{c}{Adversarial Training on AG} & \multicolumn{3}{c}{Adversarial Training on MR} \\\cmidrule(lr){2-4}\cmidrule{5-7}
\multicolumn{1}{c}{}    & TF           & BA           & \multicolumn{1}{r}{\modelc}          & TF           & BA           & \modelc       \\\midrule
Ori   & 91.9 (-0.3)  & 91.9 (-0.3)  & 91.4 (-0.8)   & 86.6 (-1.5)  & 86.7 (-1.4)  & 82.8 (-5.3)  \\
TF    & 53.0 (40.5)  & 24.0 (11.5)  & \textbf{14.5 ( 2.0)} & 28.8 (19.3)  & 8.0 (-1.5)   & \textbf{2.9 (-6.6)}  \\
PSO   & 54.1 (32.5)  & 59.5 (37.9)  & 31.4 ( 9.8)  & 18.8 (11.3)  & 12.5 ( 5.0)  & 4.7 (-2.8)   \\
BA    & 28.9 (10.5)  & 47.9 (29.5)  & 18.2 (-0.2)   & 12.7 (-1.2)  & 35.8 (21.9)  & 9.6 (-4.3)  \\
BAE   & 79.4 ( 5.8)  & 80.2 ( 6.6)  & 74.3 ( 0.7)  & 43.4 ( 5.9)  & 40.3 ( 2.8)  & 30.8 (-6.7)  \\
\modelc & \textbf{19.2 ( 4.8)}  & \textbf{19.8 ( 5.4)}  & 58.0 (43.6)  & \textbf{1.0 ( 0.4)}  & \textbf{0.6 ( 0.0)}   & 17.2 (16.6)  \\\bottomrule
\end{tabular}
\caption{After attack accuracy$\%$ on adversarially trained classifiers. Each column is an adversarially trained classifier and each row is an attack method. `Ori' means the accuracy on the original test set. The value in the parentheses show the absolute accuracy increase after the adversarial training. We highlight the most effective attack method on each classifier. See Table~\ref{tab:advtrain_other} (in Supplementary Material) for classifiers adversarially trained using BAE and PSO}\label{tab:advtrain}
\end{table*}

==> table/table_advtrain_other.tex <==
\begin{table}[htb]
\centering
\small
\begin{tabular}{r|rr|rr}
\toprule
\multicolumn{1}{l}{Attack}      & \multicolumn{2}{l}{Adversarial Training on AG} &  \multicolumn{2}{l}{Adversarial Training on MR} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\multicolumn{1}{l}{Method}   & BAE                  & \multicolumn{1}{r}{PSO}     & BAE                  & PSO             \\\midrule
Ori   & 90.8 (-1.4)          & 92.3 ( 0.1)          & 85.9 (-2.2)          & 87.8 (-0.3)         \\
TF    & \textbf{9.6 (-2.9)}           & 25.4 (12.9)     & 4.6 (-4.9)           & 22.2 (12.7)            \\
PSO   & 30.8 ( 9.2)          & 60.1 (38.5)       & 6.5 (-1.0)           & 18.1 (10.6)          \\
BA    & 33.2 (14.8)          & 27.5 ( 9.1)         & 27.8 (13.9)         & 14.4 ( 0.5)          \\
BAE   & 76.5 ( 2.9)          & 79.7 ( 6.1)         & 48.8 (11.3)          & 39.1 ( 1.6)      \\
\modelc & 19.4 ( 5.0)          & \textbf{20.8 ( 6.4)}     & \textbf{2.6 ( 2.0)}           & \textbf{0.6 ( 0.0)}       \\\bottomrule
\end{tabular}
\caption{After attack accuracy$\%$ on adversarially trained classifiers. }\label{tab:advtrain_other}
\end{table}

==> table/table_auto_metric.tex <==
\begin{table*}[htb]
\centering
\small
\begin{tabular}{r|r@{\hskip 1ex}rrr@{\hskip 2ex}r@{\hskip 1ex}r@{\hskip 1mm}r@{\hskip 1mm}r|rrrr@{\hskip 1ex}r@{\hskip 1mm}r@{\hskip 1mm}r}
\toprule
\multicolumn{1}{c}{}      & \multicolumn{8}{c}{After Attack Accuracy ($\downarrow$)}          & \multicolumn{7}{c}{GPT2 Perplexity Ratio ($\downarrow$)}        \\\cmidrule(lr){2-9}\cmidrule(lr){10-16}
\multicolumn{1}{c}{}      & Ori  & TF   & PSA  & BA   & BAE  & SCPN & ASRSu & \multicolumn{1}{c}{ASRSc} & TF   & PSA  & BA   & BAE  & SCPN & ASRSu & ASRSc \\\midrule
AG    & 92.2 & 12.5 & 21.6 & 18.4 & 73.6 & 38.0 & \textbf{11.6}  & 14.4  & 6.97 & 7.81 & 5.54 & 3.52 & 8.21 & \textbf{1.03}  & 1.07  \\
MR    & 88.1 & 9.5  & 7.5  & 13.9 & 37.5 & 29.0 & 2.2   & \textbf{0.6}   & 3.10 & 3.13 & 2.83 & 3.71 & 3.24 & \textbf{1.09}  & 1.26  \\
Yelp  & 96.5 & \textbf{4.4}  & 80.7 & 9.1  & 50.9 & 15.8 & 9.8   & 19.6  & 2.80 & 3.16 & 1.68 & 2.60 & 6.62 & \textbf{1.08}  & 1.09  \\
IMDB  & 89.8 & \textbf{6.3}  & 70.4 & 18.2 & 46.1 & 8.1  & 9.8   & 20.0  & 2.47 & 1.65 & 1.56 & 1.60 & 5.48 & 1.19  & \textbf{1.14}  \\
SNLI  & 90.7 & 3.4  & 8.0  & \textbf{1.6}  & 4.1  & 25.9 & 3.0   & 1.8   & 4.93 & 3.75 & 3.18 & 5.03 & 6.15 & \textbf{2.79}  & 2.86  \\
MNLI  & 80.8 & 5.6  & 10.9 & 2.1  & 10.3 & 18.3 & 1.2   & \textbf{0.8}   & 4.95 & 3.62 & 2.88 & 5.80 & 6.49 & 1.62  & \textbf{1.60}  \\
MNLIM & 81.9 & 4.7  & 12.6 & 2.2  & 12.6 & 16.7 & 1.8   & \textbf{1.6}   & 4.76 & 3.99 & 2.99 & 5.25 & 6.14 & \textbf{1.43}  & 1.55  \\\midrule
\multicolumn{2}{c}{} & \multicolumn{7}{c}{USE Semantic Similarity ($\uparrow$)}          & \multicolumn{7}{c}{CE Semantic Similarity ($\uparrow$)}        \\\cmidrule(lr){3-9}\cmidrule(lr){10-16}
\multicolumn{1}{r}{}      &  & TF   & PSA  & BA   & BAE  & SCPN & ASRSu & \multicolumn{1}{r}{ASRSc} & TF   & PSA  & BA   & BAE  & SCPN & ASRSu & ASRSc \\\midrule
AG    &  & 0.86 & 0.83 & 0.86 & \textbf{0.93} & 0.54 & 0.90  & 0.82  & 0.82 & 0.83 & 0.82 & 0.87 & 0.53 & 0.72  & \textbf{0.89}  \\
MR    &  & 0.83 & 0.80 & 0.85 & 0.81 & 0.55 & \textbf{0.94}  & 0.77  & 0.83 & 0.78 & 0.82 & 0.74 & 0.56 & 0.79  & \textbf{0.93}  \\
Yelp  &  & 0.91 & 0.90 & \textbf{0.94} & \textbf{0.94} & 0.26 & 0.93  & 0.86  & 0.75 & \textbf{0.78} & 0.73 & 0.77 & 0.35 & 0.59  & 0.76  \\
IMDB  &  & 0.94 & 0.94 & 0.96 & \textbf{0.98} & 0.24 & 0.94  & 0.89  & 0.74 & \textbf{0.78} & 0.74 & 0.76 & 0.32 & 0.57  & 0.71  \\
SNLI  &  & 0.70 & 0.68 & 0.78 & 0.63 & 0.56 & \textbf{0.92}  & 0.82  & 0.62 & 0.60 & 0.69 & 0.54 & 0.56 & 0.82  & \textbf{0.92}  \\
MNLI  &  & 0.80 & 0.79 & 0.86 & 0.76 & 0.62 & \textbf{0.93}  & 0.82  & 0.73 & 0.70 & 0.75 & 0.66 & 0.58 & 0.77  & \textbf{0.93}  \\
MNLIM &  & 0.81 & 0.80 & 0.86 & 0.78 & 0.63 & \textbf{0.92}  & 0.82  & 0.75 & 0.73 & 0.75 & 0.67 & 0.59 & 0.77  & \textbf{0.93}  \\\bottomrule
\end{tabular} 
\caption{Automatic metric evaluation on adversarial sentences.)}\label{tab:auto_metrics}
\end{table*}



==> table/table_auto_metric_wins.tex <==
\begin{table}
\centering\small
\begin{tabular}{rrrr@{\hskip 1ex}r@{\hskip 1ex}r}
\toprule
                            & TF & BA & BAE & \modelu & \modelc \\\midrule
After-Attack Acc.       & 16 & 15 & 0   & \textbf{20}     & 19     \\
GPT2 PPL Ratio          & 4  & 13 & 4   & \textbf{26}     & 23     \\
USE Sim.           & 9 & 20 & 12  & \textbf{22}     & 7      \\
CE Sim. & 11 & 14 & 11  & 10     & \textbf{24}    \\\bottomrule
\end{tabular}
\caption{Number of wins measured on Table~\ref{tab:auto_metrics}. We do not include PSO in computing number of wins because we fail to get results on Yelp and IMDB.}
\label{tab:auto_metric_num_wins}
\end{table}


==> table/table_cases.tex <==
\begin{table*}[t]
\centering
% \small
\begin{tabular}{p{.98\textwidth}}
\toprule
% \textbf{Original Text (Negative):} \textit{what madonna does here can't properly be called acting -- more accurately , it's moving and it's talking and it's occasionally gesturing , sometimes all at once .}\\
% \textbf{Paraphrased Text (Positive): } \textit{what madonna does here can't be called acting -- more accurately, madonna makes it moving when she wants to, and sometimes not, sometimes gesturing, sometimes all the same.}\\
% \textbf{Metric:} Editing Distance: 13, USE Cosine Sim. = 0.95, Perplexity Ratio: 0.92\\\midrule

% \textbf{Original Text (Negative):} \textit{well-nigh unendurable . . . though the picture strains to become cinematic poetry , it remains depressingly prosaic and dull .}\\
% \textbf{Paraphrased Text (Positive): } \textit{well-nigh dead-on, but even as the picture strains to become cinematic poetry, it remains sobering, prosaic and dull.}\\
% \textbf{Metric:} Editing Distance: 5, USE Cosine Sim. = 0.96, Perplexity Ratio: 0.62\\\midrule

% \textbf{Original Text (World): } \textit{US surgical strikes continue in Fallujah, Samarra, and Tal Afar. But US says Iraqi forces are not ready to launch major attacks. By Howard LaFranchi.}\\
% \textbf{Paraphrased Text (Tech): } \textit{US surgical strikes continue on Fallujah, Falluja and Tal Afar. The US and Iraqi forces are getting ready to complete the attack. By Howard LaFranchie
% }\\
% \textbf{Metric:} Editing Distance: 9, USE Cosine Sim. = 0.92, Perplexity Ratio: 0.80\\\midrule

% \textbf{Original Text (Sport): } \textit{Michael Phelps, who has won five gold  medals in the Olympic pool, said Friday he was pulling out of  Saturday's 4x100 meter medley relay final to give team mate Ian  Crocker the chance to swim.}\\
% \textbf{Paraphrased Text (World):} \textit{Michael Phelps, who has won four gold medals in an Olympic swim, was revealed to be disqualified from the men's 200-metre medley relay to try to give fellow swimmer Ian Crocker a chance...}\\
% \textbf{Metric:} Editing Distance: 20, USE Cosine Sim. = 0.92, Perplexity Ratio: 0.35\\\midrule


% \textbf{Original Text (Tech): } \textit{The world 's top mobile phone maker Nokia said on Tuesday its phones would be used in a project to test wireless public transport fares in Hanau, near Frankfurt in Germany, beginning early next year.}\\
% \textbf{Original Text (World): } \textit{The world's largest mobile phone maker Nokia said Wednesday that its technology will be used to form a new provider of public transport fares in Hanau, near Frankfurt, Germany, beginning early next year.}\\
% \textbf{Metric:} Editing Distance: 12, USE Cosine Sim. = 0.91, Perplexity Ratio: 0.75\\

\textbf{Original Text (Business):} Qualcomm Inc. on Friday raised its quarterly profit forecast due to strong demand for its mobile phone technology. The San Diego company said it expects earnings .\\
\textbf{Paraphrased Text (Sci/Tech):} Qualcomm Inc. on Friday raised its quarterly earnings forecast, reflecting a strong outlook for mobile devices, as the San Diego-based company continued growth.\\
\textbf{Metrics:} Edit distance: 14; GPT2 Perplexity ratio: 0.74; USE similarity: 0.84; CE similarity: 0.91\\
\textbf{Paraphrased Text (Sci/Tech):} Qualcomm Inc. on Friday raised its quarterly earnings forecast due to strong demand in the mobile phone market, as it looked for a higher quarterly profit.\\
\textbf{Metrics:} Edit distance: 13; GPT2 Perplexity ratio: 0.75; USE similarity: 0.91; CE similarity: 0.86\\
\textbf{Paraphrased Text (Sci/Tech):} Qualcomm Inc. plans to increase its quarterly profit forecast due to continued growth in its mobile phone business. Meanwhile, the company said it expects earnings.\\
\textbf{Metrics:} Edit distance: 11; GPT2 Perplexity ratio: 0.88; USE similarity: 0.88; CE similarity: 0.84\\\midrule

\textbf{Original Text (World):} Bangladesh is willing to sign a protocol with the United States to set up a joint working group like India and Pakistan did to enhance Dhaka 's capability to effectively deal with future terrorist acts in the country.\\
\textbf{Paraphrased Text (Business):} Bangladesh is poised to sign an agreement with the United States to create a new strategic partnership, like India and Pakistan, which highlights Dhaka's ability to help fight terrorism, terrorism, and other threats.\\
\textbf{Metrics:} Edit distance: 21; GPT2 Perplexity ratio: 0.66; USE similarity: 0.80; CE similarity: 0.90\\
\textbf{Paraphrased Text (Sports):} Bangladesh has decided to reach an agreement with the United States to set up a joint strategy between giants Pakistan and India and to support Dhaka's efforts to keep up with the tough situation in the region.\\
\textbf{Metrics:} Edit distance: 19; GPT2 Perplexity ratio: 0.95; USE similarity: 0.68; CE similarity: 0.80\\
\textbf{Paraphrased Text (Sci/Tech):} Bangladesh is willing to come to terms with the United States to set up a program, jointly with India and Pakistan, to enhance Dhaka technology as access to security technologies to prevent terrorist attacks in the country.\\
\textbf{Metrics:} Edit distance: 16; GPT2 Perplexity ratio: 1.19; USE similarity: 0.75; CE similarity: 0.90\\\midrule

\textbf{Original Text (negative):} dong never pushes for insights beyond the superficial tensions of the dynamic he's dissecting , and the film settles too easily along the contours of expectation .\\
\textbf{Paraphrased Text (positive):} dong never quite gets out of the superficiality of his film, exploring and dissecting the conflict that never takes us much beyond the contours of narrative points\\
\textbf{Metrics:} Edit distance: 20; GPT2 Perplexity ratio: 0.63; USE similarity: 0.78; CE similarity: 0.90\\\midrule

\textbf{Original Text (negative): }the good is very , very good . . . the rest runs from mildly unimpressive to despairingly awful .\\
\textbf{Paraphrased Text (positive):} the good is very, very good. and it can go, from the unimpressive, to the awful.\\
\textbf{Metrics: }Edit distance: 6; GPT2 Perplexity ratio: 0.53; USE similarity: 0.78; CE similarity: 0.90\\
\textbf{Paraphrased Text (positive):} the good is very, very good... while also ranging from very unimpressive to pretty damn awful.\\
\textbf{Metrics:} Edit distance: 6; GPT2 Perplexity ratio: 0.62; USE similarity: 0.82; CE similarity: 0.92\\

\bottomrule

\end{tabular}
\caption{Case study. We show several examples from the AG and MR datasets. }
\label{tab:case}
\end{table*}


==> table/table_datasets.tex <==
\begin{table}[htb]
\small
\centering
\begin{tabular}{cccccc}
\toprule
\textbf{Name}      & \textbf{Type} & \textbf{\#C} & \textbf{Cased} & \textbf{Train/Test} & \textbf{Len} \\
\midrule
AG & Topic & 4 & Y & 120k/7.6k  &  54     \\
MR & Sentiment & 2 & N & 9k/1k & 24\\
Yelp & Sentiment & 2 & Y & 160k/38k & 182\\
IMDB & Sentiment & 2 & Y & 25k/25k & 305\\\midrule
SNLI & NLI & 3 & Y & 570k/10k & 15/8\\
MNLI & NLI & 3 & Y & 433k/10k & 28/11\\
\bottomrule
\end{tabular}
\caption{Dataset details. \#C means number of classes. Cased means whether the dataset is cased or uncased. Len is the number of BERT word-pieces in a sentence. For the NLI dataset, the two numbers in Len represent the length for the premise and the hypothesis.}
\label{tab:dataset}
\end{table}


==> table/table_editdis.tex <==
\begin{table}[htb]
\centering
\small
\begin{tabular}{rrrrrrrr}
\toprule
      & TF   & PSA  & BA   & BAE  & SCPN & ASRSu & ASRSc \\\midrule
AG    & 5.8  & 6.4  & 4.6  & 2.1  & 13.9 & 12.8  & 13.7  \\
MR    & 3.0  & 3.3  & 2.3  & 1.9  & 8.2  & 6.0   & 9.5   \\
Yelp  & 25.2 & 27.6 & 20.9 & 27.5 & 14.5 & 54.7  & 48.8  \\
IMDB  & 49.8 & 71.1 & 46.0 & 57.0 & 18.6 & 89.4  & 81.0  \\
SNLI  & 1.4  & 1.4  & 1.2  & 1.3  & 3.6  & 2.8   & 3.8   \\
MNLI  & 1.7  & 1.6  & 1.3  & 1.5  & 4.6  & 3.7   & 4.9   \\
MNLIM & 1.8  & 1.8  & 1.3  & 1.4  & 5.0  & 4.4   & 5.8   \\\bottomrule
\end{tabular}
\caption{Edit distance metric. }\label{tab:edit_dis}
\end{table}


==> table/table_mturk.tex <==
\begin{table*}[htb]
\centering
\small
\begin{tabular}{r|rrr|rrr|rrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Label Match\% ($\uparrow$)} & \multicolumn{3}{c}{Sentence Quality ($\uparrow$)} & \multicolumn{3}{c}{Sentence Similarity ($\uparrow$)} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
\multicolumn{1}{c}{} & AG        & MR       & \multicolumn{1}{c}{SNLI}     & AG         & MR         & \multicolumn{1}{c}{SNLI}       & AG          & MR          & SNLI        \\\midrule
Ori    & 80.0      & 93.3     & 72.0     & 4.21       & 4.16       & 4.40       &             &             &             \\
TF     & 73.3 (3)          & \textbf{73.5 (1)} & 32.0 (6)          & 3.58 (3)          & 3.21 (4)          & 2.50 (5)          & 2.08 (4)          & 2.12 (3)          & 1.83 (4)          \\
PSO    & 68.0 (4)          & 64.5 (4)          & 36.5 (3)          & 3.29 (6)          & 3.51 (2)          & 3.03 (3)          & 1.92 (6)          & 1.95 (5)          & 1.59 (5)          \\
BA     & 67.0 (5)          & 69.0 (3)          & 34.5 (5)          & 3.39 (5)          & 3.20 (5)          & 2.82 (4)          & 2.02 (5)          & \textbf{2.15 (1)} & 1.85 (3)          \\
BAE    & 59.5 (6)          & 58.0 (5)          & 36.0 (4)          & 3.54 (4)          & 2.81 (6)          & 2.48 (6)          & 2.14 (2)          & 1.93 (6)          & 1.37 (6)          \\
\modelu & 79.5 (2)          & 57.5 (6)          & \textbf{50.0 (1)} & \textbf{4.33 (1)} & \textbf{3.57 (1)} & \textbf{3.26 (1)} & 2.12 (3)          & 2.14 (2)          & \textbf{2.29 (1)} \\
\modelc & \textbf{80.0 (1)} & 71.3 (2)          & 43.0 (2)          & 3.86 (2)          & 3.44 (3)          & 3.15 (2)          & \textbf{2.33 (1)} & 2.07 (4)          & 2.10 (2)   \\       
\bottomrule
\end{tabular}
\caption{MTurk experiment result. The number in the parentheses shows the rank of the method.}\label{tab:mturk}
\end{table*}

==> table/table_new_cases.tex <==
\begin{table}[tb]
\centering
\small
\begin{tabular}{p{.98\columnwidth}}
\toprule
\textbf{Ori (pos)}: a wry , affectionate delight .\\
\textbf{Adv (neg)}: a wry tale of little more than sweet affection.\\
\textbf{Adv (neg)}: laughably, affectionate.\\
\midrule
\textbf{Ori (neg)}: makes for a pretty unpleasant viewing experience .\\
\textbf{Adv (pos)}: a unpleasant experience and painful to watch.\\
\textbf{Adv (pos)}: it's an extremely uncomfortable experience to watch.\\
\bottomrule
\end{tabular}
\caption{Heterogeneous adversarial sentences found by \model on MR dataset. }
\label{tab:case_new}
\end{table}


==> table/table_traj.tex <==
\begin{table}[htb]
\small
    \centering
    \begin{tabular}{p{0.98\columnwidth}}
    \toprule
        $\bu^{(0)}$: it is still an interesting movie in its own way. \\
        $\bu^{(1)}$: it is still \red{\textbf{fascinating enough,}} in its own way. \\
        $\bu^{(2)}$: it is still fascinating enough, \red{\textbf{and on its}} way. \\
        $\bu^{(3)}$: it is still fascinating enough, and \red{\textbf{also entertaining enough}}. \\
        $\bu^{(4)}$: \red{\textbf{the film is}} fascinating enough, and also entertaining enough. \\
        $\bu^{(5)}$: the film is fascinating \red{\textbf{because it is}} also entertaining enough. \\
        $\bu^{(6)}$: the film is fascinating because \red{\textbf{the details are}} entertaining enough. \\
    \bottomrule
    \end{tabular}
    \caption{An example of running \model for 6 iterations using block size $3$. $\bu^{(0)}$ is the original sentence, and we highlight the substituted blocks in each iteration.}
    \label{tab:traj}
\end{table}

==> table_new/table_human_old.tex <==
\begin{table*}[htb]
\centering
\caption{Human Similarity Evaluation. }\label{tab:human_sim}
\begin{tabular}{rcccccc}
\toprule
           & \multicolumn{2}{c}{AG}      & \multicolumn{2}{c}{MR}      & \multicolumn{2}{c}{TREC}    \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Threshold  & 0.80         & 0.95         & 0.80         & 0.95         & 0.80         & 0.95         \\\midrule
TextFooler & 3.72 (±0.87) & 3.93 (±0.80) & 3.20 (±1.17) & 3.30 (±1.18) & 2.71 (±1.23) & 3.25 (±1.67) \\
CLARE      & 3.53 (±0.97) & 3.75 (±0.88) & 2.34 (±0.96) & 2.44 (±0.98) & 2.68 (±1.12) & 3.00 (±1.15) \\
R\&R       & 3.81 (±0.99) & 4.12 (±0.92) & 3.46 (±0.81) & 3.48 (±0.82) & 3.17 (±1.15) & 3.59 (±1.05) \\\midrule
           & \multicolumn{2}{c}{HATE}    & \multicolumn{2}{c}{FAKE}    &              &              \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Threshold  & 0.80         & 0.95         & 0.80         & 0.95         &              &              \\\midrule
TextFooler & 3.45 (±1.33) & 3.76 (±1.31) & 3.07 (±1.36) & 3.58 (±1.30) &              &              \\
CLARE      & 2.89 (±1.49) & 3.89 (±1.26) & 3.22 (±1.41) & 3.67 (±1.30) &              &              \\
R\&R       & 3.43 (±1.42) & 3.59 (±1.34) & 3.24 (±1.33) & 3.81 (±1.12) &              &              \\\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[htb]
\centering
\caption{Human Fluency Evaluation. }\label{tab:human_fluency}
\begin{tabular}{rcccccc}
\toprule
           & AG           &              & MR           &              & TREC         &              \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
           & 0.80         & 0.95         & 0.80         & 0.95         & 0.80         & 0.95         \\\midrule
TextFooler & 3.34 (±0.66) & 3.58 (±0.58) & 3.35 (±0.82) & 3.49 (±0.84) & 3.46 (±1.22) & 2.88 (±1.25) \\
CLARE      & 3.73 (±0.83) & 3.65 (±0.80) & 3.43 (±0.85) & 3.33 (±0.82) & 3.15 (±1.37) & 3.00 (±0.00) \\
R\&R       & 3.76 (±0.83) & 3.87 (±0.92) & 3.58 (±0.88) & 3.61 (±0.82) & 3.47 (±1.31) & 3.14 (±1.21) \\\midrule
           & HATE         &              & FAKE         &              &              &              \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
           & 0.80         & 0.95         & 0.80         & 0.95         &              &              \\
TextFooler & 3.28 (±1.12) & 3.61 (±1.10) & 3.23 (±1.17) & 3.53 (±1.28) &              &              \\
CLARE      & 4.13 (±0.98) & 4.41 (±0.86) & 4.40 (±0.84) & 4.47 (±0.77) &              &              \\
R\&R       & 3.89 (±1.02) & 3.94 (±0.95) & 3.88 (±1.01) & 4.17 (±0.77) &              &              \\\bottomrule
\end{tabular}
\end{table*}


\begin{table}[htb]
\centering
\caption{Human Label Match Evaluation. }\label{tab:human_match}
\begin{tabular}{lllllllll}
\toprule
           & AG   &      & MR   &      & TREC &      & HATE &      \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
           & 0.80 & 0.95 & 0.80 & 0.95 & 0.80 & 0.95 & 0.80 & 0.95 \\\midrule
TextFooler & 0.96 & 0.9  & 0.85 & 0.92 & 0.58 & 0.88 & 0.59 & 0.46 \\
CLARE      & 0.93 & 0.93 & 0.68 & 0.74 & 0.71 & 0.75 & 0.65 & 0.81 \\
R\&R       & 0.97 & 0.99 & 0.8  & 0.85 & 0.77 & 0.89 & 0.72 & 0.76 \\\bottomrule
\end{tabular}
\end{table}
